Beyond Value-Function Gaps: Improved Instance-Dependent Regret Bounds for Episodic Reinforcement Learning

We provide improved gap-dependent regret bounds for reinforcement learning in finite episodic Markov decision processes. Compared to prior work, our bounds depend on alternative definitions of gaps. These definitions are based on the insight that, in order to achieve a favorable regret, an algorithm does not need to learn how to behave optimally in states that are not reached by an optimal policy. We prove tighter upper regret bounds for optimistic algorithms and accompany them with new information-theoretic lower bounds for a large class of MDPs. Our results show that optimistic algorithms can not achieve the information-theoretic lower bounds even in deterministic MDPs unless there is a unique optimal policy.

==> commands.tex <==
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\Ecal}{\mathcal{E}}

\newcommand{\E}{\mathbb{E}}

\newtheorem{lemma}{Lemma}[section]
% \newtheorem{figur}[lemma]{Figure}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{example}[lemma]{Example}
\newtheorem{exercise}[lemma]{Exercise}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{fig}[lemma]{Figure}
\newtheorem{tab}[lemma]{Table}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{test}{Lemma}
\newtheorem{conj}[lemma]{Conjecture}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{assumption}[lemma]{Assumption}

\newcommand{\minimize}[3]{
& \underset{#1}{\operatorname{minimize}}
& & #2\\
& \operatorname{s.t.}
& & #3
}

\newcommand{\maximize}[3]{
& \underset{#1}{\textrm{maximize}}
& & #2\\
& \textrm{s.t.}
& & #3
}

% Arg<x>
\DeclareMathOperator*{\argmin}{arg\,min} % * Places subscript directly under operator
\DeclareMathOperator*{\argmax}{arg\,max}             
\DeclareMathOperator*{\arginf}{arg\,inf} 
\DeclareMathOperator*{\argsup}{arg\,sup} 
\DeclareMathOperator*{\Span}{span}
\DeclareMathOperator{\gap}{gap}
\DeclareMathOperator{\clip}{clip}
\newcommand*{\one}{{\bf 1}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\II}{\mathbb{I}} % Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\LL}{\mathbb{L}} % Loss
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\ZZ}{\mathbb{Z}} % Integers
\newcommand{\XX}{\mathbb{X}} %
\newcommand{\YY}{\mathbb{Y}} %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Zcal}{\mathcal{Z}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Ocal}{\mathcal{O}}

\newcommand{\w}{\mathbb{w}}

==> main_body/alt_upper_bounds.tex <==
\section{Novel upper bounds for optimistic algorithms}
\label{sec:upper_bounds}
Before presenting improved our upper bounds for general MDPs, we first discuss and state our results for the special case when transitions are deterministic to motivate our definitions in the more general stochastic transition case.

\subsection{Special case: Markov decision processes with deterministic transitions}

As hinted to in the introduction, the way in which prior regret bounds treat value-function gaps independently at each state-action pair can lead to excessively loose regret bounds. 
Prior regret bounds~\citep{simchowitz2019non,lykouris2019corruption,jin2020simultaneously}  that use value-function gaps
scale at least as
$$\sum_{s,a \colon \gap(s,a) >0 } \frac{H\log(K)}{\gap(s,a)} + 
\sum_{s,a \colon \gap(s,a) =0 }
\frac{H\log(K)}{\gap_{\min}} \quad \textrm{ where }\quad  \gap_{\min} = \!\!\!\min_{s, a \colon \gap(s,a) > 0}\! \gap(s,a).
$$ 
To illustrate where these bounds are loose, let us revisit the example MDP in \pref{fig:summary}. Here, the bounds evaluate to $  \frac{H\log(K)}{c}+\frac{H\log(K)}{\epsilon}+\frac{SH\log(K)}{\epsilon}$, where the first two terms come form the positive gaps and the last term comes from all the state-action pairs with zero gaps which are accounted for with $1 / \gap_{\min}$. There are several places for improvement:
\begin{enumerate}[label = \textbf{P.\arabic*}]
\item\label{enum_prob_1} \textbf{State-action pairs that can only be visited by taking optimal actions:} We should not pay the $1/\gap_{\min}$ factor for such $(s,a)$ as there are no other suboptimal policies $\pi$ to distinguish from $\pi^*$ in such states.
    \item\label{enum_prob_3} 
    \textbf{State-action pairs that can only be visited by taking at least one suboptimal action:}
    We should not pay the $1 / \gap(s_2, a_3)$ factor for state-action pair $(s_2, a_3)$ and the $1 / \gap_{\min}$ factor for $(s_2, a_4)$ because no optimal policy visits $s_2$. Such state-action pairs should only be accounted for with the price to learn that $a_2$ is not optimal in state $s_1$. After all,  learning to distinguish between $\pi_1$ and $\pi_2$ is unnecessary for optimal return.
\end{enumerate}

\ref{enum_prob_1} and \ref{enum_prob_3} suggest that the price at which a state-action pair $(s,a)$ occurs in the regret bound should not only be determined by the rewards achievable after visiting $(s,a)$ or $s$, as is the case in value function gaps $\gap(s,a) = V^*(s) - Q^*(s,a)$. Therefore, in addition to the value function gap which measures how much reward to go is lost by playing $a$ instead of the optimal action in $s$, we also consider the difference of entire sum of rewards. In particular, we look at the difference of optimal return $v^*$ and the return $v^*_{s,a}$ of the best suboptimal policy that visits $(s,a)$,
\begin{align*}
v^* - v^{*}_{s,a} \qquad \textrm{where} \qquad
v^{*}_{s,a} \equiv \max_{\substack{\pi \in \Pi \setminus \Pi^* \colon\\ w^\pi(s,a) > 0}}  v^\pi~.
\end{align*}
The intuition behind this term is that $v^* - v^{*}_{s,a}$ measures the cost 

\paragraph{Regret bounds for deterministic transition MDPs.} 
We now interpret \pref{def:return_gap} for deterministic MDPs and derive a novel regret bound which is essentially tight for optimistic algorithms. For any state-action pair $(s,a)$ let $\pi^\dagger_{(s,a)}$ denote the policy with highest value function which is not an optimal policy. Formally $\pi^\dagger_{(s,a)} = \argmin_{\pi: (s,a)\in\pi, \pi\not\in \Pi^*}v^* - v^\pi$. \pref{def:return_gap} now evaluates to $\returngap(s,a) = \gap(s,a) + \frac{v^* - v^{\pi^\dagger_{(s,a)}}}{H}$ and Theorem~\ref{thm:reg_bound_gen_informal} yields the following regret bound.
\begin{corollary}
\label{cor:det_trans_reg}
Assume \textsc{StrongEuler} is applied to an MDP with deterministic transitions and optimal value function bounded by $1$. Then its regret is bounded with high probability for all $K \geq 1$ as
\begin{align*}
    \regret(K) &\leq O\Bigg(\sum_{s,a \colon \returngap(s,a)> 0} \frac{H\log(K)}{v^* - v^{\pi^\dagger_{(s,a)}}}\Bigg).
\end{align*}
\end{corollary}
We now compare this bound again to the existing bound stated in \pref{eq:cor_1b_simchowitz}. In \citet{simchowitz2019non}, $\alpha \in [0,1]$ is defined as the smallest value such that for all $(s,a,s') \in \Scal\times\Acal\times\Scal$ it holds that
$P(s'|s,a) - P(s'|s,\pi^*(s)) \leq \alpha P(s'|s,a)$, where $\pi^*$ is a Bellman-optimal policy.
Hence, unless all state-action pairs are optimal it must hold that $\alpha=1$. For any $\gap(s,a)>0$ it holds that $v^* - v^{\pi^\dagger_{(s,a)}} \geq \sum_{(s',a') \in v^{\pi^\dagger_{(s,a)}}}\gap(s',a') \geq \gap(s,a)$. Further for every $(s,a) \in \Zcal_{opt}$ for which $\returngap(s,a) >0$ it holds that $v^* - v^{\pi^\dagger_{(s,a)}} \geq \gap_{\min}$. Combining these two observations it holds that the bound in Corollary~\ref{cor:det_trans_reg} is no worse than the one in \citep{simchowitz2019non}.
We would further like to emphasize that this bound achieves the $O(SH \log(K) / c)$ regret we hoped to achieve in the example MDP in Figure~\ref{fig:summary}. 

is addressed by the fact that at any episode, to reach states only visited by an optimal policy we have had to play an optimal policy and hence we have not incurred any regret during the respective episode. This observation can actually be taken a little further and allows us to not include state-action pairs $(s,a)\in \Scal\times\Acal$ such that $\gap(s,a) = 0$ and all preceding state-action pairs in the topology of the MDP also have zero gaps. This observation will also motivate our formal definition of the return gap, $\returngap$.
Problem~\ref{enum_prob_3} is %and \ref{enum_prob_2} are
addressed in a slightly more subtle manner. 
Our intuition for deterministic MDPs is the following and is based on the gap decomposition for the instantaneous regret with respect to any suboptimal policy $\pi$:
\begin{align*}
    v^* - v^{\pi} = \sum_{h=1}^H \gap(s_h^{\pi},a_h^{\pi}).
\end{align*}
In the above $(s_h^{\pi},a_h^{\pi})$ is the state-action pair visited by $\pi$ at layer $h$. We can replace the gap at each state-action pair in the support of $\pi$ by a normalized sum (by $H$) of all strictly positive gaps at states in the support of $\pi$ while still preserving the regret decomposition of $v^* - v^{\pi}$. This suggests that the regret we have to pay at every $(s,a)\in\pi$ is actually dependent on $(v^* - v^{\pi})/H$ rather than $\gap(s,a)$ (in fact it turns out we can take the maximum of the two quantities). 
\subsection{General case: Markov decision processes with stochastic transitions}
Our intuition can be extended to arbitrary MDPs by replacing the normalized sum by an appropriate expectation.
Formally we define the return gaps as
\begin{definition}[Return gap]
\label{def:return_gap}
For any state-action pair $(s,a)\in\Scal\times\Acal$ let $\Bcal(s,a)\equiv \{B \leq \kappa(s), S_{\kappa(s)} = s, A_{\kappa(s)} = a\}$ denote the event that state-action pair $(s,a)$ is visited and that a suboptimal action was played any time up to visiting $(s,a)$. 
We define the return gap as
\begin{align*}
    \returngap(s,a) \equiv \gap(s,a)\lor\min_{\substack{\pi \in \Pi \colon \\\PP_{\pi}(\Bcal(s,a)) > 0}}&~
    \frac{1}{H}
    \EE_{\pi}\left[ \sum_{h=1}^H \gap(S_h, A_h) ~ \bigg| ~\Bcal(s,a) \right]
    %\\
    % = \gap(s,a)\lor\min_{\substack{\pi \in \Pi \colon \\\PP_{\pi}(\Bcal(s,a)) > 0}}&~
    %\frac{1}{H}
    %\EE_{\pi}\left[ \sum_{h=1}^{\kappa(s)} \gap(S_h, A_h) ~ \bigg| ~\Bcal(s,a) \right],
\end{align*}
if there is a policy $\pi \in \Pi$ with $\PP_\pi(\Bcal(s,a)) > 0$ and $\returngap(s,a) \equiv 0$ otherwise. %\cd{is the case here missed too easily?}
\end{definition}
%\tm{I am not sure why the second equality holds.} \cd{Since we are minimizing over all policies, the minimum would always be attained at a policy that acts optimal from $(s,a)$ on.}

The intuition behind event $\Bcal(s,a)$ follows from what we discussed regarding Problem~\ref{enum_prob_1}. In particular if the event does not occur, then we have followed an optimal policy $\pi^*$ up to and including $(s,a)$, and hence no regret has been incurred. The benefit of $\Bcal(s,a)$ is apparent in non-deterministic MDPs. Consider the case when we are faced with a policy $\pi$ which with probability $1-\delta$ follows $\pi^*$ and with probability $\delta$ visits some highly sub-optimal state action pair $(s,a)$ at which $\gap(s,a)$ is large. Taking the expected sum of gaps, rather than conditioning on $\Bcal(s,a)$ would result in a regret bound which $\gap(s,a)$ by $\delta$, effectively using $v^* - v^{\pi}$ as the gap. The event $\Bcal$ allows us to only pay a cost inversely proportional to $\returngap(s,a) \geq \gap(s,a)$. Our (informal) main upper bound pertains to the \textsc{StrongEuler} algorithm proposed in~\citep{simchowitz2019non} and is stated below.
\begin{theorem}[Informal]
\label{thm:reg_bound_gen_informal}
The regret $\regret(K)$ of  \textsc{StrongEuler} is bounded with high probability as 
\begin{align*}
    \regret(K) &\lessapprox \sum_{\substack{(s,a)\in\Scal\times\Acal \colon \\\returngap(s,a) > 0}} \frac{\Vcal^*(s,a)}{\returngap(s,a)}
    \log\frac{MK}{\delta}
    %+ \sum_{s,a} SH^3 \log\frac{MK}{\delta} \min\left\{ \log \frac{MK}{\delta}, \log \frac{MH}{\returngap(s,a)}\right\}
     \quad + \quad SAH^3 (S \vee H)\log \frac{MH}{\returngap_{\min}} \log\frac{MK}{\delta}
    .
\end{align*}
\end{theorem}
In the above $\Vcal^*(s,a)$ is a term capturing the variance of the $Q$ function of $\pi^*$ at $(s,a)$ and we have restricted the bound to only the terms which have inverse polynomial dependence on the gaps. \tm{We could include discussion about the bound here or defer to the end of the next subsection as it is now.}

\paragraph{Comparison with existing gap-dependent bounds.} We now proceed to compare our bound  to the existing gap-dependent bound for \textsc{StrongEuler} in \citet[Corollary B.1]{simchowitz2019non}
\begin{align}
\label{eq:cor_1b_simchowitz}
    \regret(K) \leq O\Bigg(\sum_{(s,a) \notin \Zcal_{opt}} \frac{\alpha H\Vcal^*(s,a)\log(K)}{\gap(s,a)} + |\Zcal_{opt}|\frac{H\Vcal^*\log(K)}{\gap_{\min}}\Bigg),
\end{align}
where $\Vcal^* = \max_{(s,a)}\Vcal^*(s,a)$ and $\Zcal_{opt} = \{ s, a \colon \gap(s,a) = 0\}$ is the set state-action pair with zero $\gap(s,a) = 0$ according to a Bellman optimal policy $\pi^*$.
We here focus only on terms that have a dependency on $K$ and an inverse-polynomial dependency on gaps as all other terms are comparable. Our bound in \pref{thm:reg_bound_gen_informal} is no worse than this bound by noting that on $\Zcal_{opt}$ it always holds that $\returngap(s,a) \geq \frac{\gap_{\min}}{H}$. Further, outside of $\Zcal_{opt}$ our bound has no dependence on $H$ and $\returngap(s,a) \geq \gap(s,a)$.
However, to see that our bound can be much tighter, consider the case where a state $s\in \Zcal_{opt}$ is only reachable after making suboptimal actions, i.e., where the sum of value-function gaps is much larger than $\gap_{\min}$. By our definition of return gaps, we only pay the inverse of these larger gaps instead of $\gap_{\min}$.
This improvement is already apparent in our motivating example in Figure~\ref{fig:summary} where \pref{thm:reg_bound_gen_informal} achieves the desired $\log(K)/c$ regret bound as opposed to the $\log(K)/\epsilon$ bound suggested by prior work. 





\subsection{Improved clipping: from minimum gap to average gap}
\label{sec:gen_clipping}
We now sketch how to derive our regret guarantees for \textsc{StrongEuler}. Our framework is also applicable to other algorithms that are \emph{optmistic}, that is at every episode they maintain a Q-function, $\bar Q_k$, which overestimates the Q-function of $\pi^*$ on every state-action pair, $\bar Q_k(s,a) \geq Q^*(s,a)$, with high probability.
We would like to point out that our results match the ones in \citep{simchowitz2019non} without requiring \emph{strong optimism}.
% Strongly optimistic algorithms maintain upper-confidence bounds $\bar V_k$ and $\bar Q_k$ for each episode $k$ that satisfy $\bar Q_k  \geq Q^*$ and $\bar V_k \geq V^*$ for all $k$ with high probability.
Strongly optimistic algorithms are optimistic and they further guarantee that their surpluses which, roughly speaking, quantify the local amount of optimism in $s,a$ and formally defined as
\begin{align}
\label{eq:surpl_def}
    E_k(s,a) = \bar Q_k(s,a) - r(s,a) - \langle P(\cdot|s,a), \bar V_k\rangle,
\end{align}
are guaranteed to be non-negative as well (with high probability).

We now formalize how to exchange the gap at each state-action pair for the return gap. We begin by quickly recalling the key steps in existing analyses.
At the core of gap-dependent analyses is the following bound on the instantaneous regret by the \emph{clipped surpluses}

\begin{align*}
    V^*(s_1) - V^{\pi_k}(s_1) \lessapprox \sum_{s,a} w^{\pi_k}(s,a)\clip[E_{k}(s,a) \vert \gap(s,a) \lor \gap_{\min}],
\end{align*}
where $\clip[ a | b] = \indicator{a \geq b} a$ is the clipping operator.
This is tighter than the usual bound achievable by just using optimism and the definition of surpluses which is $V^*(s_1) - V^{\pi_k}(s_1) \leq \sum_{(s,a) \in \Scal\times\Acal}w_{\pi_k}(s,a)E_{k}(s,a)$ and is the key to the instance dependent bounds.
% First, using optimism and the definition of surpluses one can show that the instantaneous regret at episode $k$ is bounded by the surpluses as $V^*(s_1) - V^{\pi_k}(s_1) \leq \sum_{(s,a) \in \Scal\times\Acal}w_{\pi_k}(s,a)E_{k}(s,a)$. Next, we observe, that using a self-bounding trick together with the fact that $V^*(s_1) - V^{\pi_k}(s_1) = \sum_{(s,a) \in \Scal\times\Acal}w_{\pi_k}(s,a)\gap(s,a)$, we can bound $V^*(s_1) - V^{\pi_k}(s_1) \leq \sum_{(s,a) \in \Scal\times\Acal}w_{\pi_k}(s,a)E_{k}(s,a)$.
Next, using concentration arguments it is possible to show that $E_{k}(s,a) \lessapprox \sqrt{\frac{\Vcal(s,a)}{k}}$, for sub-optimal state-action pairs which are visited often, where $\Vcal(s,a)$ is a variance term for $(s,a)$. We can intuitively ignore other state-action pairs as they do not generate too much regret. This implies that we can not incur regret for more than $\frac{\Vcal(s,a)}{(\gap(s,a)\lor \gap_{\min})^2}$ rounds as otherwise we would have $\sqrt{\frac{\Vcal(s,a)}{\sum_{j=1}^k w_{\pi_j}(s,a)}} < \gap(s,a)\lor \gap_{\min}$, which implies that $E_k(s,a)$ would be clipped to zero.

\paragraph{Improving on $\gap_{\min}$.}
The issues described with prior work upper bounds occur precisely because of clipping to $\gap_{\min}$. Suppose we replaced $\gap_{\min}$ with a generic clipping function $\epsilon_{k} :\Scal\times\Acal \rightarrow \mathbb{R}$. How large can we hope for this function to be? The following self-bounding trick reveals some intuition. By definition of gaps we can write $\frac{1}{4}(V^*(s_1) - V^{\pi_k}(s_1))  = \frac{1}{4}\sum_{(s,a)\in\Scal\times\Acal} w_{\pi_k}(s,a)\gap(s,a) =  \frac{1}{4}\EE_{\pi_k}[\sum_{h=1}^H\gap(S_h,A_h)]$. By definition of surpluses and optimism we also have an upper bound on the instantaneous regret as $V^*(s_1) - V^{\pi_k}(s_1) \leq \sum_{h=1}^H\EE_{\pi_k}[ E_k(S_h,A_h)]$. Subtracting $\frac{1}{4}(V^*(s_1) - V^{\pi_k}(s_1))$ from both sides implies $\frac{3}{4}(V^*(s_1) - V^{\pi_k}(s_1)) \leq \sum_{h=1}^H\EE_{\pi_k}\left[\clip[E_k(S_h,A_h)|\frac{1}{4}\gap(S_h,A_h)]\right]$. Further, if we were able to lower bound $\EE_{\pi_k}[\sum_{h=1}^H\gap(S_h,A_h)]$ by our clipping function as $\sum_{h=1}^H\EE_{\pi_k}[\gap(S_h,A_h)] \geq \sum_{h=1}^H\EE_{\pi_k}[\epsilon_{k}(S_h)]$ we could repeat the self bounding trick again and arrive at the desired $V^*(s_1) - V^{\pi_k}(s_1) \leq 4\sum_{h=1}^H\EE_{\pi_k}\left[\clip[E_k(S_h,A_h)|\frac{1}{4}(\gap(S_h,A_h)]\lor \epsilon_{k}(S_h))\right]$. Thus the key in deriving improved regret bounds is to lower bound the expected sum of gaps as tightly as possible by the clipping function. The above discussion is made formal by the next proposition.

\begin{restatable}[Improved surplus clipping bound]{proposition}{surplusclippingbound}
\label{prop:surplus_clipping_bound}
Let the surpluses $E_k(s,a)$ be generated by a strongly optimistic algorithm and consider clipping thresholds $\epsilon_k \colon \Scal \times \Acal \rightarrow \RR^+_0$ that satisfy
\begin{align*}
    \EE_{\pi_k}\left[\sum_{h=B}^H \epsilon_k(S_h, A_h) \right]
    \leq \frac{1}{2} \EE_{\pi_k} \left[\sum_{h=1}^H \gap(S_h, A_h) \right]
\end{align*}
where $B = \min\{ h \in [H+1] \colon \gap(S_h, A_h) > 0 \}$ is the first time a non-zero gap was encountered.
Then the instantaneous regret of $\pi_k$ can be bounded as
\begin{align*}
    V^*(s_1) - V^{\pi_k}(s_1) 
    \leq 4 \sum_{s,a} w^{\pi_k}(s,a) \clip\left[ E_k(s,a) ~\bigg| ~ \frac 1 4 \gap(s,a) \vee \epsilon_{k}(s, a) \right].
\end{align*}
\end{restatable}

We now make the quick observation that taking $\epsilon_{k} \equiv \frac{\gap_{\min}}{2H}$ will satisfy the condition of Proposition~\ref{prop:surplus_clipping_bound}, because on the event $\Bcal$ there exists at least one positive gap in the sum $\sum_{h=1}^H\gap(S_h,A_h)$, which, by definition, is at least $\gap_{\min}$. This shows that our results already can recover the bounds in prior work, with significantly less effort. The condition in Proposition~\ref{prop:surplus_clipping_bound} suggests that one can set $\epsilon_{k}(S_h,A_h)$ proportional to the average expected gap under policy $\pi_k$. Formally, the clipping function we use is 
\begin{align}
    \epsilon_{k}(s,a) = 
    \frac{1}{2H}
    \EE_{\pi_k}\left[ \sum_{h=1}^H \gap(S_h, A_h) ~ \bigg| ~\Bcal(s,a)\right]. %+ \indicator{\PP_{\pi_k}[\Acal_{H+1}^c | S_{\kappa(s)} = s] = 1}\infty
    \label{eqn:epsilon_choice}
\end{align}

In the corner case where the event $\Bcal$ has zero probability under $\pi_k$, we set $\epsilon_{k}(s,a) = \infty$. 
\pref{lem:clipping_gaps_rel} in \pref{app:upper_bounds} shows that the above definition satisfies the condition in \pref{prop:surplus_clipping_bound}. 
This definition is also never worse than the minimum-gap clipping of existing analysis since $\epsilon_{k}(s,a) \geq \frac{\gap_{\min}}{2H}$ follows from the fact that in event $\Bcal$ at least one gap is non-zero. 
% (\pref{lem:clipping_lower_bound} in \pref{app:upper_bounds}).
Further, $\epsilon_{k}(s,a)$ takes a simple form in MDPs with deterministic transitions: $\epsilon_{k}(s,a) = \frac{1}{2H}\sum_{s\in supp(\pi_k)}\gap(s,\pi_k(s)) = \frac{\return{*}-\return{\pi_k}}{2H}$, if $(s,a) \in \pi_k$ and $\epsilon_{k}(s,a)=\infty$ otherwise (because $\Bcal$ has zero probability).




\subsection{Policy-dependent regret bound for \textsc{StrongEuler}}
We will now show how our results from the previous sections translate into a stronger regret bound on the concrete example of \textsc{StrongEuler}. Ignoring lower-order terms, \citet{simchowitz2019non} showed that the surpluses of this algorithm are bounded as $E_k(s,a) \lessapprox \sqrt{\frac{\Vcal^*(s,a)\log(\bar n_k(s,a))}{\bar n_k(s,a)}}$ where $\bar n_k(s,a) = \sum_{j=1}^{k-1} w^{\pi_j}(s,a)$ are the expected number of samples for $(s,a)$ up to episode $k$ and $\Vcal^*(s,a) = \VV[R(s,a)] + \VV_{s'\sim P(\cdot|s,a)}[V^{*}(s')]$ is the one-step variance term w.r.t. the optimal value function. \pref{prop:surplus_clipping_bound} with the clipping to the average gap gives in this case
\begin{equation}
    \label{eq:reg_bound_fake}
    \begin{aligned}
        &\regret(K) 
        \lessapprox \sum_{k=1}^K\sum_{s,a} w^{\pi_k}(s,a)\clip\left[\sqrt{\frac{\Vcal^*(s,a)\log(\bar n_k(s,a))}{\bar n_k(s,a)}} ~\bigg|~ \gap(s,a) \lor \epsilon_{k}(s,a)\right].
    \end{aligned}
\end{equation}
% Here, we denote the choice of optimal policy in the gap for episode $k$ as $\pi^*_k$. 
Existing analysis now translate such a clipping bound into a $\log(K)$ regret bound using an integration argument \citep[e.g. ][]{dann2019policy,simchowitz2019non}. However, we cannot rely on these arguments since our clipping thresholds are not necessarily constant across episodes. To address this technical challenge, we derive the following lemma based on an optimization view on such terms
\begin{lemma}\label{lem:opt_lemma_simpler}
For any sequence of thresholds $\gamma_1, \dots \gamma_K > 0$, consider the problem with $x_0 = 1$
\begin{align*}
    \underset{x_1, \dots x_K \in [0,1]}{\operatorname{maximize}}
    \sum_{k=1}^K \frac{ x_k\sqrt{\log(\sum_{j=0}^k x_j)}}{\sqrt{\sum_{j=0}^k x_j}}
    \quad \mathrm{s.t.~~ for~~ all~~ }k \in [K]: \quad 
    \frac{\sqrt{\log(\sum_{j=0}^k x_j)}}{\sqrt{\sum_{j=0}^k x_j}} \geq \gamma_k.
\end{align*}
The optimal value is bounded for any $t \in [K]$ from above as
$\frac{\log(t)}{\epsilon_t} + \sqrt{(K-t) \log K}$.
\end{lemma}
Applying this lemma for each $(s,a)$ with $x_k = w^{\pi_k}(s,a)$ and appropriate clipping thresholds $\gamma_k \approx (\gap(s,a) + \epsilon_{k}(s,a))/\sqrt{\Vcal^*(s,a)}$ we can derive our main result:

\begin{theorem}[Informal]
% \label{thm:reg_bound_gen_informal}
The regret $\regret(K)$ of \texttt{StrongEuler} is bounded with high probability as
\begin{align*}
    \regret(K) \lessapprox
    \sum_{s,a} \min_{t \in [K_{(s,a)}]} \left\{
    \frac{\Vcal^*(s,a)}{\gap(s,a) + \epsilon_{t}(s,a)}
    + \sqrt{\Vcal^*(s,a) (K_{(s,a)} - t)}\right\} \log(K),
    %O\Bigg(\log(K)\max_{\pi_{1:K}}\min_{\pi^*_{1:K}}\sum_{(s,a) \in \Scal\times\Acal} \min_{t\in %[K]}\Bigg\{\frac{\Vcal_{\max_t}(s,a)}{\breve \gap_{\pi_t}^{\pi^*_t}(s,a)} + %\sum_{k=t+1}^K\frac{\Vcal_{\max_k}(s,a)}{\sum_{j=t+1}^k \breve %\gap_{\pi_j}^{\pi^*_j}(s,a)}\Bigg\}\Bigg).
\end{align*}
where we only show terms with (inverse-)polynomial dependency on gaps and $K_{(s,a)}$ is the last episode during which a policy supported on $(s,a)$ was played. For the full bound, see \pref{thm:reg_bound_gen_se} in the appendix.
\end{theorem}
\tm{Possibly state the full version of the result here as we already have an informal version above.}
Note that our regret bound depends through $\epsilon_{t}(s,a)$, the average gap encountered by $\pi_t$, on the policies that the algorithm played. Note that this dependency is generally mild and can be removed by taking a maximum over all possible policies $\pi_t$ (see discussion on deterministic MDPs for an example).

Our regret bound can smoothly interpolate between the worst-case rate of $\sqrt{K}$ achieved for $t \ll K$ when all gaps and average gaps are $O(\sqrt{\Vcal^*(s,a) K})$ and the gap-dependent regret rate achieved when $t \approx K$ that scales inversely with gaps. Note that our bound depends on the gaps in all episodes and can benefit from choices for $t$ that yields a large gap or average gap in the late episodes.



==> main_body/intro.tex <==
\section{Introduction}

Reinforcement Learning (RL) is a general scenario where learners, or agents, interact with
the environment to achieve some goal. The environment and an agent's interactions
are typically modeled as a Markov decision process (MDP) \citep{puterman1994markov},
which can represent a rich variety of tasks. But, for which MDPs can an agent or an RL algorithm succeed? This requires a theoretical analysis of the complexity of an MDP.
This paper studies this question in the tabular episodic setting, where an agent interacts with the environment in episodes of fixed length $H$ and where the size of the state and action space is finite ($S$ and $A$ respectively).

While the performance of RL algorithms in tabular Markov decision processes has been 
the subject of many studies in the past \citep[e.g.][]{fiechter1994efficient,kakade2003sample,osband2013more,dann2015sample,dann2017unifying,azar2017minimax,jin2018q,zanette2019tighter, dann2019strategic}, the vast majority of existing analyses focuses on worst-case problem-independent regret bounds, which only take into account the size of the MDP, the horizon $H$ and the number of episodes $K$. 
% Only recently, 
%As the practical success of RL systems grows in various settings such as board games, computer games and robotics so does the theoretical understanding of the underlying principles. The performance of RL systems is usually measured by the incurred regret, i.e., the difference in reward between the selected policies and the optimal policy. One formal paradigm for studying RL systems is through modelling them as Markov Decision Processes (MDPs). Our work focuses on the tabular setting, where we assume that the set of states $\Scal$ and the set of actions $\Acal$ both have finite cardinality, $S$ and $A$ respectively. Further, we assume a finite horizon $H$, episodic setting consisting of $K$ episodes.
%
%Majority of prior work in this setting has focused on deriving min-max optimal regret bounds which have sub-linear dependence on the time horizon $T = HK$. Very recently,

Recently, however, some significant progress has been achieved towards deriving
more optimistic problem-dependent guarantees. This includes 
more refined regret bounds for the tabular episodic setting that depend on 
structural properties of the specific MDP considered \citep{simchowitz2019non, lykouris2019corruption, jin2020simultaneously}. Motivated by instance-dependent analyses in multi-armed bandits \citep{lai1985asymptotically}, these analyses derive 
gap-dependent regret-bounds of the form 
    $O\left(\sum_{(s,a)\in\Scal\times\Acal} \frac{H\log(K)}{\gap(s,a)}\right)$,
    where the sum is over state-actions pairs $(s, a)$ and
    where the gap notion is defined as the difference of the optimal value function $V^{*}$ of the Bellman optimal policy $\pi^*$ and the $Q$-function of $\pi^*$ at a sub-optimal action:
    $\gap(s,a) = V^{*}(s) - Q^{*}(s,a)$. We will refer to this gap definition as \emph{value-function gap} in the following. We note that a similar notion of gap has been used in the infinite horizon setting to achieve instance-dependent bounds \citep{auer2007logarithmic,tewari2008optimistic,auer2009near,filippi2010optimism,ok2018exploration}, however, a strong assumption about irreducability of MDP is required.
    The actual regret bounds are more complicated and include additional $(s, a)$-dependent factors that only depend on the rewards-to-go from $(s,a)$ and that are therefore irrelevant to this discussion.

While this notion of gap generalizes that of the multi-armed bandit setting, we argue that it has a major limitation: each gap only depends on the rewards-to-go from the state-action pair and does not take into account how this state-action pair can be reached. Hence, existing gap-dependent regret bounds treat all state-action pairs equally and ignore their topological ordering in the MDP which can have a major impact on the performance of RL. In this paper, we address this issue and formalize the following key observation about the difficulty of RL in an episodic MDP through improved instance-dependent regret bounds:
\begin{center}
\begin{minipage}{0.9\linewidth}
\emph{Learning a policy with optimal return does not require an RL agent to distinguish between actions with similar outcomes (small value-function gap) in states that can only be reached by taking highly suboptimal actions (large value-function gap).}
%\emph{To learn an optimal policy, an RL agent does not need to learn to distinguish between actions with similar outcomes (small value-function gap) in states that can only be reached by taking highly suboptimal actions (large value-function gap).}
\end{minipage}
\end{center}

To illustrate this insight, consider autonomous driving, where each episode corresponds to driving from a start to a destination. If the RL agent decides to run a red light on a crowded intersection, then a car crash is inevitable. Even though the agent could slightly affect the severity of the car crash by steering, this effect is small and, hence, a good RL agent does not need to learn how to best steer after running a red light. Instead, it would only need a few samples to learn to obey the traffic light in the first place as the action of disregarding a red light has a very large value-function gap.

%a self-driving car. Every episode of the learning problem is driving along a pre-determined route and every time step in an episode is a traffic condition to which we should react. For example if the car reaches a red light it should stop. Suppose, however, that the car decides to choose the action of continuing in the red light state. The value gap at such a state-action pair must be large, as this is clearly a sub-optimal action. After this action is executed, all of the following state-action pairs are most likely equally bad e.g., the car might decide to stop in the middle of the red light intersection, or maybe it decides to drive around and avoid other cars. In any case the result is most likely a car accident. Due to this each of the value gaps for state-action pairs after running the red light are small as there is not much difference between the optimal policy and a sub-optimal one in terms of the final result. Treating the post red light states as equal now implies we should pay high regret, however, we know that a real-world system would need very few examples to learn to obey the traffic light signal.

\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\centerline{\includegraphics[scale=.7]{imgs/gap_example_tikz.pdf}}
\end{minipage}
\resizebox{.7\textwidth}{!}{\begin{minipage}{1\textwidth}
\begin{tabular}{l|l|}
\cline{2-2}
 & Regret bounds for deterministic transition MDPs: \\ \hline
\multicolumn{1}{|l|}{Prior work:} & $R_{prior}(K) \leq O\big(\sum_{(s,a) \not\in\pi^*} \frac{H\log(K)}{\gap(s,a)}\big)$                        \\ \hline
\multicolumn{1}{|l|}{This work:}  & $R_{our}(K) \leq O\bigg(\sum_{(s,a) \not\in\pi^*} \frac{H\log(K)}{\return{*} - \return{\pi^*_{(s,a)}}}\bigg)$ \\ \hline
\multicolumn{1}{|l|}{Comparison:} & $\return{*} - \return{\pi^*_{(s,a)}} = \sum_{(s',a') \in \pi^*_{(s,a)}\setminus \pi^*} \gap(s',a')$       \\ \hline
\end{tabular}
\end{minipage}}
\caption{Illustration of the limitations of existing gap-dependent bounds for episodic Markov decision processes}
\label{fig:summary}
\end{figure}

To understand how this observation translates into regret bounds,  consider the small MDP  in \prettyref{fig:summary}. The MDP has deterministic transitions and only terminal rewards. There are two decision points, $s_1$ and $\tilde s$, with two actions each, and all other states have only a single action. There are only three policies in this MDP: $\pi^*$, which plays action $a_1$ in state $s_1$ and then proceeds along the red path; $\pi_1$, which takes action $a_2$ at $s_1$ and $a_3$ at $\tilde s$ and proceeds along the blue path; and $\pi_3$ which takes action $a_2$ at $s_1$ and $a_4$ at $\tilde s$. All state-action pairs have zero reward except for the state-action pairs in the final layer. These rewards are illustrated in the figure in their respective colors and imply $V^{\pi^*}(s_1) > V^{\pi_1}(s_1) > V^{\pi_2}(s_1)$, $\gap(s_1,a_2) = c$ and $\gap(\tilde s,a_4) = \epsilon$ where $\epsilon \ll c$. Finally, the Bellman optimality condition implies that $\pi^*(\tilde s) = a_3$. On all other states the gap is zero. The idea behind the gap-dependent bounds is now to capture the necessary, from an information theoretic perspective, number of rounds to distinguish $\pi^*$ from any other sub-optimal $\pi$ on all states $s \in \Scal$. In the example MDP of \pref{fig:summary}, this amounts to distinguishing $\pi_1$ from $\pi^*$ on state $s_1$ and $\pi_2$ from $\pi_1$ in state $\tilde s$. Thus, the accumulated regret would be of the order $O(\log(T)(1/c + 1/\epsilon))$. However, a reasonable algorithm would only need to determine that $a_2$ is a sub-optimal action at state $s_1$, which would eliminate both $\pi_1$ and $\pi_2$ after only $\log(T)/c^2$ rounds. The incurred regret would then be only $O(\log(T)/c)$. Notice that $\epsilon$ 
and $c$ can be selected arbitrarily in this example. In particular, if we take $c=0.5$ and 
$\epsilon = 1/\sqrt{K}$ this bound remains only logarithmic in the number of episodes, while 
the recently derived gap-dependent regret bounds scale with $\sqrt{K}$.

This work is motivated by the insight and observations just discussed.
Our  main contributions are two-fold. First, we investigate in what episodic 
MDPs an algorithm could benefit from that insight by deriving information-theoretic regret lower-bounds. We show that existing gap-dependent bounds indeed cannot be improved in problems where each state is visited by an optimal policy with some probability. However, we also prove a new lower bound when the transitions of the MDP are deterministic that depends on a new notion of gap, called \emph{total-return gap}, and which indicate that a more favorable regret may be possible to achieve when there are states outside of the support of optimal policies.

%the information theoretic limits for certain classes of MDPs, which include the example in \pref{fig:fail_gap} and show that any algorithm will incur regret at least $\Omega(\log(T)/c)$.
Second, we show that improved regret bounds are indeed possible by proving a tighter regret bound for \textsc{StrongEuler}, an existing algorithm based on the optimism-in-the-face-of-uncertainty (OFU) principle \citep{simchowitz2019non}. While it is difficult to give a closed-form expression of our bound for general stochastic MDPs, we can express our bound in terms of return gaps in problems with deterministic transitions. 
In fact, we show that it matches our lower-bound up to factors in the episode length $H$.
Our results suggest that value-function gaps are not sufficient to capture all the relevant problem structure that determines the regret of RL agents and that new forms of regret bounds are necessary. They also show that, at least for some MDPs, return gaps provide a finer alternative for quantifying the difficulty of episodic RL. %already incur regret at most $O(\log(T)/c)at the above example, and in general incur smaller regret, than what has been shown. 
%\cd{bring back bullet list? Are our contributions sufficiently clear?}
%n summary, our contributions are:
%\begin{enumerate}
%    \item to derive closed form regret lower bounds for deterministic transitions MDPs whenever the value function of any policy does not exceed the maximum reward on any state-action pair,
%    \item to derive closed form regret lower bounds for MDPs in which $\pi^*$ has non-zero probability to visit every state $s\in\Scal$ and the value function of any policy does not exceed the maximum reward on any state-action pair,
%    \item and we show improved upper bounds, which do not suffer from the small-gap problem we described above, for established optimistic algorithms.
%\end{enumerate}

%\cd{Should we already show here an example of a simple MDP where value function gaps are too much to illustrate the main point of the paper?}

%\cd{Can we summarize our results in a nice table -- like Table~\ref{tab:summary}?}






==> main_body/relatedwork.tex <==
\section{Additional related work}

% Gap-dependent analyses in episodic MDPs \citet{simchowitz2019non,lykouris2019corruption, yang2020q, jin2020simultaneously}, maybe \citet{du2020agnostic}?
%Min-max rates for Reinforcement Learning in the tabular setting are relatively well established by now both in the infinite horizon setting, for communicating MDPs \citep{auer2009near,bartlett2012regal,osband2016lower}, and in the finite horizon case \citep{osband2013more,dann2015sample,dann2017unifying,azar2017minimax,jin2018q,zanette2019tighter,simchowitz2019non}. The lower bounds in the infinite horizon setting are in the order of $\Omega(\sqrt{DSAT})$, where $D$ is a measure of the diameter of the MDP. Upper bounds for this setting are of the order $\tilde O(DS\sqrt{AT})$. \citet{agrawal2017optimistic} manage to show $\tilde O(D\sqrt{SAT})$ for large $T$. In the finite horizon setting the established min-max rate is $\tilde\Theta(H\sqrt{SAK})$.

Instance dependent bounds for the simpler problem of MAB were first introduced in \citet{lai1985asymptotically}. The techniques were very recently generalized and simplified in the work of \citet{garivier2019explore}. \citet{graves1997asymptotically} extend the lower bounds to the setting of controlled Markov chains with infinite horizon and proposed an algorithm which achieves the bound asymptotically. Building on their work \citet{combes2017minimal} establish both lower and (asymptotic) upper bounds for the Structured Stochastic Bandit problem. For infinite horizon MDPs with additional assumptions the works of \citet{auer2007logarithmic,tewari2008optimistic,auer2009near,filippi2010optimism,ok2018exploration} establish logarithmic in horizon regret bounds of the form $O(D^2S^2A\log(T)/\delta)$, where $\delta$ is a gap-like quantity and $D$ is a diameter measure. \citet{tewari2008optimistic,ok2018exploration} propose asymptotically optimal algorithms based on a linear program (LP). Their regret upper bounds can also be converted to have a gap-like flavor. Very recently there has been a plethora of papers proposing instance dependent regret bounds for finite horizon tabular MDPs~\citep{simchowitz2019non,lykouris2019corruption, yang2020q, jin2020simultaneously,du2020agnostic}. All of these bounds scale at least as $\Omega(SH\log(T)/\gap_{\min})$. The dependence on number of actions in the above works scales with better gap-dependent factors than $1/\gap_{\min}$. \citet{simchowitz2019non} show an MDP instance on which no optimistic algorithm can hope to do better.

==> main_body/upper_bounds.tex <==
\section{Novel upper bounds for optimistic algorithms}
\label{sec:upper_bounds}

As hinted to in the introduction, the way prior regret bounds treat value-function gaps independently at each state-action pair can lead to excessively loose guarantees.
Bounds  that use value-function gaps \citep{simchowitz2019non,lykouris2019corruption,jin2020simultaneously}
scale at least as
$$\sum_{s,a \colon \gap(s,a) >0 } \frac{H\log(K)}{\gap(s,a)} + 
\sum_{s,a \colon \gap(s,a) =0 }
\frac{H\log(K)}{\gap_{\min}} ,
$$ 
where state-action pairs with zero gap appear, with  $\gap_{\min} = \min_{s, a \colon \gap(s,a) > 0} \gap(s,a)$, the smallest positive gap.
To illustrate where these bounds are loose, let us revisit the example in \pref{fig:summary}. Here, these bounds evaluate to $  \frac{H\log(K)}{c}+\frac{H\log(K)}{\epsilon}+\frac{SH\log(K)}{\epsilon}$, where the first two terms come from state-action pairs with positive value-function gaps and the last term comes from all the state-action pairs with zero gaps. There are several opportunities for improvement:
\begin{enumerate}[label = \textbf{O.\arabic*}]
    \item\label{enum_prob_1} \textbf{State-action pairs that can only be visited by taking optimal actions:} We should not pay the $1/\gap_{\min}$ factor for such $(s,a)$ as there are no other suboptimal policies $\pi$ to distinguish from $\pi^*$ in such states.
    \item\label{enum_prob_3} 
    \textbf{State-action pairs that can only be visited by taking at least one suboptimal action:}
    We should not pay the $1 / \gap(s_2, a_3)$ factor for state-action pair $(s_2, a_3)$ and the $1 / \gap_{\min}$ factor for $(s_2, a_4)$ because no optimal policy visits $s_2$. Such state-action pairs should only be accounted for with the price to learn that $a_2$ is not optimal in state $s_1$. After all,  learning to distinguish between $\pi_1$ and $\pi_2$ is unnecessary for optimal return. 
\end{enumerate}
Both opportunities suggest that the price $\frac{1}{\gap(s,a)}$ or $\frac{1}{\gap_{\min}}$ that each state-action pair $(s,a)$ contributes to the regret bound can be reduced by taking into account the regret incurred by the time $(s,a)$ is reached. Opportunity~\ref{enum_prob_1} postulates that if no regret can be incurred up to (and including) the time step $(s,a)$ is reached, then this state-action pair should not appear in the regret bound. Similarly, if this regret is necessarily large, then the agent can learn this with few observations and stop reaching $(s,a)$ earlier than $\gap(s,a)$ may suggest. Thus, as claimed in \ref{enum_prob_3}, the contribution of $(s,a)$ to the regret should be more limited in this case.

Since the total regret incurred during one episode by a policy $\pi$ is simply the expected sum of value-function gaps visited (\pref{lem:gap_decomp_pi} in the appendix),
\begin{align}
v^* - v^\pi = \EE_{\pi}\left[ \sum_{h=1}^H \gap(S_h, A_h) \right],
\label{eq:reg_decomp}
\end{align}
we can measure the regret incurred up to reaching $(S_{t}, A_{t})$ by the sum of value function gaps $\sum_{h=1}^t \gap(S_h, A_h)$ up to this point $t$. We are interested in the regret incurred up to visiting a certain state-action pair $(s,a)$ which $\pi$ may visit only with some probability. We therefore need to take the expectation of such gaps conditioned on the event that $(s,a)$ is actually visited. We further condition on the event that this regret is nonzero, which is exactly the case when the agent encounters a positive value-function gap within the first $\kappa(s)$ time steps. We arrive at
\begin{align*}
\EE_{\pi}\left[ \sum_{h=1}^{\kappa(s)} \gap(S_h, A_h) ~ \bigg| ~S_{\kappa(s)} = s, A_{\kappa(s)} = a, B \leq \kappa(s) \right],
\end{align*}
where $B = \min \{ h \in [H+1] \colon \gap(S_h, A_h) > 0\}$ is the first time a non-zero gap is visited. This quantity measures the regret incurred up to visiting $(s,a)$ through suboptimal actions. If this quantity is large for all policies $\pi$, then a learner will stop visiting this state-action pair after few observations because it can rule out all actions that lead to $(s,a)$ quickly. Conversely, if the event that we condition on has zero probability under any policy, then $(s,a)$ can only be reached through optimal action choices (including $a$ in $s$) and incurs no regret. This motivates our new definition of gaps that combines value function gaps with the regret incurred up to visiting the state-action pair:
%Opportunity~\ref{enum_prob_1} is addressed by the fact that at any episode, to reach states only visited by an optimal policy we have had to play an optimal policy and hence we have not incurred any regret during the respective episode. This observation can actually be taken a little further and allows us to not include state-action pairs $(s,a)\in \Scal\times\Acal$ such that $\gap(s,a) = 0$ and all preceding state-action pairs in the topology of the MDP also have zero gaps. This observation will also motivate our formal definition of the return gap, $\returngap$.
%Problem~\ref{enum_prob_3} is %and \ref{enum_prob_2} are
%addressed in a slightly more subtle manner. 
%Our intuition for deterministic MDPs is the following and is based on the gap decomposition for the instantaneous regret with respect to any suboptimal policy $\pi$:
%\begin{align*}
%    v^* - v^{\pi} = \sum_{h=1}^H \gap(s_h^{\pi},a_h^{\pi}).
%\end{align*}
%In the above $(s_h^{\pi},a_h^{\pi})$ is the state-action pair visited by $\pi$ at layer $h$. We can replace the gap at each state-action pair in the support of $\pi$ by a normalized sum (by $H$) of all strictly positive gaps at states in the support of $\pi$ while still preserving the regret decomposition of $v^* - v^{\pi}$. This suggests that the regret we have to pay at every $(s,a)\in\pi$ is actually dependent on $(v^* - v^{\pi})/H$ rather than $\gap(s,a)$ (in fact it turns out we can take the maximum of the two quantities). Our intuition can be extended to arbitrary MDPs by replacing the normalized sum by an appropriate expectation. Formally we define the return gaps as follows.
\begin{definition}[Return gap]
\label{def:return_gap}
For any state-action pair $(s, a)\in\Scal\times\Acal$ define $\Bcal(s,a)\equiv \{B \leq \kappa(s), S_{\kappa(s)} = s, A_{\kappa(s)} = a\}$, where $B$ is the first time a non-zero gap is encountered. $\Bcal(s,a)$ denotes the event that state-action pair $(s,a)$ is visited 
and that a suboptimal action was played at any time up to visiting $(s,a)$.
We define the return gap as
\begin{align*}
    \returngap(s,a) \equiv \gap(s,a)\lor\min_{\substack{\pi \in \Pi \colon \\\PP_{\pi}(\Bcal(s,a)) > 0}}&~
    \frac{1}{H} \,
    \EE_{\pi} \bracket*{ \sum_{h = 1}^{\kappa(s)} \gap(S_h, A_h) ~ \bigg| ~\Bcal(s,a) }
    %\\
    % = \gap(s,a)\lor\min_{\substack{\pi \in \Pi \colon \\\PP_{\pi}(\Bcal(s,a)) > 0}}&~
    %\frac{1}{H}
    %\EE_{\pi}\left[ \sum_{h=1}^{\kappa(s)} \gap(S_h, A_h) ~ \bigg| ~\Bcal(s,a) \right],
\end{align*}
if there is a policy $\pi \in \Pi$ with $\PP_\pi(\Bcal(s,a)) > 0$ and $\returngap(s,a) \equiv 0$ otherwise. %\cd{is the case here missed too easily?}
\end{definition}
%\tm{I am not sure why the second equality holds.} \cd{Since we are minimizing over all policies, the minimum would always be attained at a policy that acts optimal from $(s,a)$ on.}

%The intuition behind event $\Bcal(s,a)$ follows from what we discussed regarding Problem~\ref{enum_prob_1}. In particular if the event does not occur, then we have followed an optimal policy $\pi^*$ up to and including $(s,a)$, and hence no regret has been incurred. The benefit of $\Bcal(s,a)$ is apparent in non-deterministic MDPs. Consider the case when we are faced with a policy $\pi$ which with probability $1-\delta$ follows $\pi^*$ and with probability $\delta$ visits some highly sub-optimal state-action pair $(s,a)$ at which $\gap(s,a)$ is large. Taking the expected sum of gaps, rather than conditioning on $\Bcal(s,a)$ would result in a regret bound which has as $\frac{1}{\delta\gap(s,a)}$ dependence, effectively using $v^* - v^{\pi}$ as the gap. Conditioning on $\Bcal(s,a)$ results in a regret bound which is only inversely proportional to $\returngap(s,a) \geq \gap(s,a) \gg \delta\gap(s,a)$. 
The additional $1/H$ factor in the second term is a required normalization suggesting that it is the average gap rather than their sum that matters.
Equipped with this definition, we are ready to state our main upper bound which pertains to the \textsc{StrongEuler} algorithm proposed by \citet{simchowitz2019non}.
\begin{theorem}[Main Result (Informal)]
\label{thm:reg_bound_gen_informal}
The regret $\regret(K)$ of  \textsc{StrongEuler} is bounded with high probability for all number of episodes $K$ as
\begin{align*}
    \regret(K) &\lessapprox \sum_{\substack{(s,a)\in\Scal\times\Acal \colon \\\returngap(s,a) > 0}} \frac{\Vcal^*(s,a)}{\returngap(s,a)}
    \log K
    %+ \sum_{s,a} SH^3 \log\frac{MK}{\delta} \min\left\{ \log \frac{MK}{\delta}, \log \frac{MH}{\returngap(s,a)}\right\}
    % \quad + \quad SAH^3 (S \vee H)\log \frac{MH}{\returngap_{\min}} \log\frac{MK}{\delta}
    .
\end{align*}
\end{theorem}
In the above, 
% $\Vcal^*(s,a)$ is a term capturing the variance of the $Q$ function of $\pi^*$ at $(s,a)$ and 
we have restricted the bound to only those terms that have inverse polynomial dependence on the gaps. % \tm{We could include discussion about the bound here or defer to the end of the next subsection as it is now.}

\paragraph{Comparison with existing gap-dependent bounds.} We now compare our bound to the existing gap-dependent bound for \textsc{StrongEuler} by \citet[Corollary B.1]{simchowitz2019non}
\begin{align}
\label{eq:cor_1b_simchowitz}
    \regret(K) \lessapprox \sum_{\substack{(s,a)\in\Scal\times\Acal \colon \\\gap(s,a) > 0}} \frac{ H\Vcal^*(s,a)}{\gap(s,a)}\log K + \sum_{\substack{(s,a)\in\Scal\times\Acal \colon \\\gap(s,a) = 0}} \frac{H\Vcal^*}{\gap_{\min}}\log K .
\end{align}
% where $\Vcal^* = \max_{(s,a)}\Vcal^*(s,a)$.
We here focus only on terms that admit a dependency on $K$ and an inverse-polynomial dependency on gaps as all other terms are comparable. 
Most notable is the absence of the second term of \pref{eq:cor_1b_simchowitz} in our bound in \pref{thm:reg_bound_gen_informal}. Thus, while state-action pairs with $\returngap(s, a) = 0$ do not contribute to our regret bound, they appear with a $1/\gap_{\min}$ factor in existing bounds. Therefore, our bound addresses \ref{enum_prob_1} because it does not pay for state-action pairs that can only be visited through optimal actions.
Further, state-action pairs that do contribute to our bound satisfy $\frac{1}{\returngap(s,a)} \leq \frac{1}{\gap(s,a)} \wedge \frac{H}{\gap_{\min}}$ and thus never contribute more than in the existing bound in \pref{eq:cor_1b_simchowitz}. Therefore, our regret bound is never worse. 
In fact, it is significantly tighter when there are states that are only reachable by taking severely suboptimal actions, i.e., when the average value-function gaps are much larger than $\gap(s,a)$ or $\gap_{\min}$. By our definition of return gaps, we only pay the inverse of these larger gaps instead of $\gap_{\min}$.
Thus, our bound also addresses \ref{enum_prob_3} and achieves the desired $\log(K)/c$ regret bound in the motivating example of \pref{fig:summary} as opposed to the $\log(K)/\epsilon$ bound of prior work. 

\paragraph{Regret bound when transitions are deterministic.}
We now interpret \pref{def:return_gap} for MDPs with deterministic transitions and derive an alternative form of our bound in this case.  
Let $\Pi_{s,a}$ be the set of all policies that visit $(s,a)$ and have taken a suboptimal action up to that visit, that is,
$$
\Pi_{s,a} \equiv \curl*{\pi \in \Pi ~\colon s^\pi_{\kappa(s)} = s ,a^\pi_{\kappa(s)} = a, \exists~ h \leq \kappa(s), \gap(s^\pi_{h},a^\pi_{h})>0}.
$$
where $(s^\pi_1, a^{\pi}_1, s^\pi_2, \dots, s^\pi_H, a^{\pi}_H)$ are the state-action pairs visited (deterministically) by $\pi$.
Further,  let $v^{*}_{s,a} = \max_{\pi \in \Pi_{s,a}} v^\pi$ be the best return of such policies.
%of the best polLet $\pi^\dagger_{(s,a)}$ denote the policy with highest value function visiting $(s,a)$ among all policies in $\Pi(s,a)$. Formally $\pi^\dagger_{(s,a)} = \argmin_{\pi \in \Pi(s,a)}v^* - v^\pi$. 
\pref{def:return_gap} now evaluates to $\returngap(s,a) = \gap(s,a) \vee \frac{1}{H}(v^* - v^{*}_{s,a})$ and the bound in  \pref{thm:reg_bound_gen_informal} can be written as
%\begin{corollary}
%\label{cor:det_trans_reg}
%Assume \textsc{StrongEuler} is run with an MDP with deterministic transitions and optimal value function bounded by $1$. Then its regret is bounded with high probability for all $K \geq 1$ as
\begin{align}
\label{eq:det_trans_reg}
    \regret(K) &\lessapprox \sum_{s,a \colon \Pi_{s,a} \neq \varnothing} \frac{H\log(K)}{v^* - v^*_{s,a}}~.
\end{align}
We show in \pref{app:unique_opt_pol}, that it is possible to further improve this bound when the optimal policy is unique by only summing over state-action pairs which are not visited by the optimal policy.
%\end{corollary}
%We now compare this bound again to the existing bound stated in \pref{eq:cor_1b_simchowitz}. In \citet{simchowitz2019non}, $\alpha \in [0,1]$ is defined as the smallest value such that for all $(s,a,s') \in \Scal\times\Acal\times\Scal$ it holds that
%$P(s'|s,a) - P(s'|s,\pi^*(s)) \leq \alpha P(s'|s,a)$, where $\pi^*$ is a Bellman-optimal policy.
%Hence, unless all state-action pairs are optimal it must hold that $\alpha=1$. For any $\gap(s,a)>0$ it holds that $v^* - v^{\pi^\dagger_{(s,a)}} \geq \sum_{(s',a') \in v^{\pi^\dagger_{(s,a)}}}\gap(s',a') \geq \gap(s,a)$. Further for every $(s,a) \in \Zcal_{opt}$ for which $\returngap(s,a) >0$ it holds that $v^* - v^{\pi^\dagger_{(s,a)}} \geq \gap_{\min}$. Combining these two observations it holds that the bound in Corollary~\ref{cor:det_trans_reg} is no worse than the one in \citep{simchowitz2019non}.
%We would further like to emphasize that this bound achieves the $O(SH \log(K) / c)$ regret we hoped to achieve in the example MDP in Figure~\ref{fig:summary}. 
%\cd{It seems that $\pi^\dagger_{(s,a)}$ is not well defined when the state can only be visited by optimal policies}

%\cd{We also seem to loose a bit of power here because there may be a policy that is optimal up to $(s,a)$ but then takes an action with a tiny gap afterwards. We would pay for this gap here instead of the smallest gap possible before reaching $(s,a)$}



\subsection{Regret analysis with improved clipping: from minimum gap to average gap}
\label{sec:gen_clipping}
In this section, we present the main technical innovations of our tighter regret analysis.
Our framework applies to \emph{optimistic} algorithms that maintain a $Q$-function estimate, $\bar Q_k(s,a)$, which overestimates the optimal $Q$-function $Q^*(s,a)$ with high probability in all states $s$, actions $a$ and episodes $k$. \cd{Are we sure we don't need strong optimism?}
We first give an overview of gap-dependent analyses and then describe our approach.

\paragraph{Overview of gap-dependent analyses. }
A central quantity in regret analyses of optimistic algorithms are \emph{surpluses} $E_k(s,a)$ which, roughly speaking, quantify the local amount of optimism in $(s, a)$ and are formally defined as
\begin{align}
\label{eq:surpl_def}
    E_k(s,a) = \bar Q_k(s,a) - r(s,a) - \langle P(\cdot|s,a), \bar V_k\rangle~.
\end{align}
Worst-case regret analyses bound the regret in episode $k$ as
$\sum_{(s,a) \in \Scal\times\Acal}w_{\pi_k}(s,a)E_{k}(s,a)$, the expected surpluses under the optimistic policy $\pi_k$ executed in that episode. Instead, gap-dependent analyses rely on a tighter version and bound the instantaneous regret by the \emph{clipped surpluses} \citep[e.g. Proposition 3.1][]{simchowitz2019non}
\begin{align}
    V^*(s_1) - V^{\pi_k}(s_1) \leq 2e \sum_{s,a} w^{\pi_k}(s,a)\clip\left[E_{k}(s,a) ~\bigg\vert~ \frac{1}{4H}\gap(s,a) \lor \frac{\gap_{\min}}{2H}\right].
    \label{eqn:old_surplusclipping}
\end{align}
% where $\clip[ a | b] = \indicator{a \geq b} a$ is the clipping operator that sets $a$ to zero if it is smaller than $b$. 
Using concentration arguments one can show that $E_{k}(s,a)$ shrinks at a rate of $\sqrt{\frac{1}{n_k(s,a)}}$, with $n_k(s,a)$ the current number of times $(s,a)$ has been visited. Thus, roughly speaking, after  $\left(\frac{\gap(s,a)\lor \gap_{\min}}{H}\right)^{-2}$ visits to $(s,a)$, the surplus falls below the threshold and does not contribute any more to the regret. Since each visit incurs at most $\frac{\gap(s,a)\lor \gap_{\min}}{H}$ regret, this leads to a $\frac{H}{\gap(s,a)\lor \gap_{\min}}$ dependency on gaps for each state-action pair.


\paragraph{Sharper clipping with general thresholds.}
Our main technical contribution for achieving a regret bound in terms of return gaps $\returngap(s,a)$ is the following improved surplus clipping bound:

\begin{restatable}[Improved surplus clipping bound]{proposition}{surplusclippingbound}
\label{prop:surplus_clipping_bound}
Let the surpluses $E_k(s,a)$ be generated by an optimistic algorithm.
Then the instantaneous regret of $\pi_k$ is bounded as follows:
\vspace{-1mm}
\begin{align*}
    V^*(s_1) - V^{\pi_k}(s_1) 
    \leq 4 \sum_{s,a} w^{\pi_k}(s,a) \clip\left[ E_k(s,a) ~\bigg| ~ \frac 1 4 \gap(s,a) \vee \epsilon_{k}(s, a) \right]~, 
\end{align*}
\vspace{-1mm}
where $\epsilon_k \colon \Scal \times \Acal \rightarrow \RR^+_0$ 
is any clipping threshold function that satisfies
\vspace{-1mm}
\begin{align*}
    \EE_{\pi_k}\left[\sum_{h=B}^H \epsilon_k(S_h, A_h) \right]
    \leq \frac{1}{2} \EE_{\pi_k} \left[\sum_{h=1}^H \gap(S_h, A_h) \right].
\end{align*}
% with $B = \min\{ h \in [H+1] \colon \gap(S_h, A_h) > 0 \}$ the first time a non-zero gap is encountered.

\end{restatable}
Compared to previous surplus clipping bounds in \eqref{eqn:old_surplusclipping}, there are several notable differences. First, instead of $\gap_{\min}/2H$, we can now pair $\gap(s,a)$ with more general clipping thresholds $\epsilon_k(s,a)$, as long as their expected sum over time steps after the first non-zero gap was encountered is at most half the expected sum of gaps. We will provide some intuition for this condition below. Note that $\epsilon_{k}(s,a) \equiv \frac{\gap_{\min}}{2H}$ satisfies the condition because the LHS evaluates to $\frac{\gap_{\min}}{2H} \PP_{\pi_k}( B \leq H)$ and there must be at least one positive gap in the sum $\sum_{h=1}^H\gap(S_h,A_h)$ on the RHS in event $\{B \leq H\}$. Thus our bound recovers existing results.
%
In addition, the first term in our clipping thresholds is $\frac{1}{4}\gap(s,a)$ instead of $\frac{1}{4H}\gap(s,a)$. \citet{simchowitz2019non} are able to remove this spurious $H$ factor only if the problem instance happens to be a bandit instance and the algorithm satisfies a condition called \emph{strong optimism} where surpluses have to be non-negative. Our analysis does not require such conditions and therefore generalizes these existing results.\footnote{Our layered state space assumption affects the $H$ dependencies in lower-order terms in our final regret compared to \citet{simchowitz2019non}. However, \pref{prop:surplus_clipping_bound} directly applies to their setting without any penalty in $H$.} 



\paragraph{Intuition for threshold condition in \pref{prop:surplus_clipping_bound}.}
The key to proving \pref{prop:surplus_clipping_bound} is the following self-bounding trick for the instantaneous regret $V^*(s_1) - V^{\pi_k}(s_1)$. The self-bounding trick works in the following way. If we have a $\rho > 0$ which is upper bounded by $\gamma \geq \rho$ and lower bounded by $0 < \beta \leq \rho$, we can further bound $(1 - c) \rho \leq \gamma - c\beta$ for any constant $c \in [0,1]$. We can now use this trick twice with $\rho = V^*(s_1) - V^{\pi_k}(s_1)$, $\gamma = \EE_{\pi_k}[\sum_{h=1}^H E_k(S_h,A_h)]$, $c=1/4$ and $\beta$ equal to either the expected sum of gaps or the assumed lower bound with clipping functions, that is $\beta = \EE_{\pi_k}[\sum_{h=1}^H \gap(S_h,A_h)]$ or $\beta=\EE_{\pi_k}[\sum_{h=1}^H \epsilon_k(S_h,A_h)]$. This implies that one half of the instantaneous regret is bounded as
\begin{align*}
    \frac{1}{2}(V^*(s_1) - V^{\pi_k}(s_1)) \leq \sum_{h=1}^H \EE_{\pi_k}\left[E_k(S_h,A_h) - \frac{\gap(S_h,A_h) + \epsilon_k(S_h,A_h)}{4}\right].
\end{align*}
Using the fact that the $\clip$ operator satisfies $a - b \leq \clip[a | b]$ gives the desired statement. This implies that, in order to achieve the tightest regret bound, we should clip $E_k(S_h,A_h)$ to the largest possible value. Thus, the goal is to lower bound the expected sum of gaps as tightly as possible by the clipping function.
Besides this insight, introducing the stopping time $B$ in the condition is key to addressing \ref{enum_prob_1} and requires a careful treatment laid out in the full proof in \pref{app:upper_bounds}.
%\cd{This is quite dense, especially without displayed equations. I am not sure how useful this is to the reader. Can we simplify this?}  By definition of gaps we can write $\frac{1}{4}(V^*(s_1) - V^{\pi_k}(s_1))  = \frac{1}{4}\sum_{(s,a)\in\Scal\times\Acal} w_{\pi_k}(s,a)\gap(s,a) =  \frac{1}{4}\EE_{\pi_k}[\sum_{h=1}^H\gap(S_h,A_h)]$. By definition of surpluses and optimism we also have an upper bound on the instantaneous regret as $V^*(s_1) - V^{\pi_k}(s_1) \leq \sum_{h=1}^H\EE_{\pi_k}[ E_k(S_h,A_h)]$. Subtracting $\frac{1}{4}(V^*(s_1) - V^{\pi_k}(s_1))$ from both sides implies $\frac{3}{4}(V^*(s_1) - V^{\pi_k}(s_1)) \leq \sum_{h=1}^H\EE_{\pi_k}\left[\clip[E_k(S_h,A_h)|\frac{1}{4}\gap(S_h,A_h)]\right]$. Further, if we were able to lower bound $\EE_{\pi_k}[\sum_{h=1}^H\gap(S_h,A_h)]$ by our clipping function as $\sum_{h=1}^H\EE_{\pi_k}[\gap(S_h,A_h)] \geq \sum_{h=1}^H\EE_{\pi_k}[\epsilon_{k}(S_h)]$ we could repeat the self bounding trick again and arrive at the desired $V^*(s_1) - V^{\pi_k}(s_1) \leq 4\sum_{h=1}^H\EE_{\pi_k}\left[\clip[E_k(S_h,A_h)|\frac{1}{4}(\gap(S_h,A_h)]\lor \epsilon_{k}(S_h))\right]$. Thus the key in deriving improved regret bounds is to lower bound the expected sum of gaps as tightly as possible by the clipping function. 

\paragraph{Choice of clipping thresholds for return gaps.}
The condition in \pref{prop:surplus_clipping_bound} suggests that one can set $\epsilon_{k}(S_h,A_h)$ to be proportional to the average expected gap under policy $\pi_k$: 
\begin{align}
    \epsilon_{k}(s,a) = 
    \frac{1}{2H}
    \EE_{\pi_k}\left[ \sum_{h=1}^H \gap(S_h, A_h) ~ \bigg| ~\Bcal(s,a)\right].
    \label{eqn:epsilon_choice}
\end{align}
if $\PP_{\pi_k}(\Bcal(s,a)) > 0$ and  $\epsilon_{k}(s,a) = \infty$ otherwise.  
\pref{lem:clipping_gaps_rel} in \pref{app:upper_bounds} shows that this choice indeed satisfies the condition in \pref{prop:surplus_clipping_bound}. 
If we now take the minimum over all policies for $\pi_k$, then we can proceed with the standard analysis and derive our main result in \pref{thm:reg_bound_gen_informal}. However, by avoiding the minimum over policies, we can derive a stronger regret bound that depends on the actual policies executed by the algorithm. We present this bound in the next section.



\subsection{Policy-dependent regret bound}
We will now show how our results from the previous sections translate into a stronger regret bound on the concrete example of \textsc{StrongEuler}. Ignoring lower-order terms, \citet{simchowitz2019non} showed that the surpluses of this algorithm are bounded as $E_k(s,a) \lessapprox \sqrt{\frac{\Vcal^*(s,a)\log(\bar n_k(s,a))}{\bar n_k(s,a)}}$ where $\bar n_k(s,a) = \sum_{j=1}^{k-1} w^{\pi_j}(s,a)$ are the expected number of samples for $(s,a)$ up to episode $k$ and $\Vcal^*(s,a) = \VV[R(s,a)] + \VV_{s'\sim P(\cdot|s,a)}[V^{*}(s')]$ is the one-step variance term w.r.t.\ the optimal value function. In this case, \pref{prop:surplus_clipping_bound} with the clipping to the average gap gives:
\begin{equation}
    \label{eq:reg_bound_fake}
    \begin{aligned}
        &\regret(K) 
        \lessapprox \sum_{k=1}^K\sum_{s,a} w^{\pi_k}(s,a)\clip\left[\sqrt{\frac{\Vcal^*(s,a)\log(\bar n_k(s,a))}{\bar n_k(s,a)}} ~\bigg|~ \gap(s,a) \lor \epsilon_{k}(s,a)\right].
    \end{aligned}
\end{equation}
% Here, we denote the choice of optimal policy in the gap for episode $k$ as $\pi^*_k$. 
An existing analysis now translates such a clipping bound into a $\log(K)$ regret bound using an integration argument \citep[e.g.][]{simchowitz2019non}. However, we cannot rely on these arguments since our clipping thresholds may not be constant across episodes. To address this technical challenge, we derive the following lemma based on an optimization view on such terms
\begin{lemma}\label{lem:opt_lemma_simpler}
For any sequence of thresholds $\gamma_1, \dots \gamma_K > 0$, consider the problem with $x_0 = 1$
\vspace{-2mm}
\begin{align*}
    \underset{x_1, \dots x_K \in [0,1]}{\operatorname{maximize}}
    \sum_{k=1}^K x_k\sqrt{\frac{ \log \paren*{\sum_{j = 0}^k x_j} }{\sum_{j=0}^k x_j}}
    \quad \mathrm{s.t.~~ for~~ all~~ }k \in [K]: \quad 
    \sqrt{\frac{\log \paren*{\sum_{j = 0}^k x_j}}{\sum_{j = 0}^k x_j}} \geq \gamma_k.
\end{align*}
\vspace{-3mm}
The optimal value is bounded for any $t \in [K]$ from above as
$\frac{\log(t)}{\epsilon_t} + \sqrt{(K-t) \log K}$.
\end{lemma}
Applying this lemma for each $(s,a)$ with $x_k = w^{\pi_k}(s,a)$ and appropriate clipping thresholds $\gamma_k \approx (\gap(s,a) \vee \epsilon_{k}(s,a))/\sqrt{\Vcal^*(s,a)}$ we can derive our main result:

\begin{theorem}
% \label{thm:reg_bound_gen_informal}
When \texttt{StrongEuler} is run with confidence parameter $\delta$, then with probability at least $1 - \delta$, its regret is bounded for all number of episodes $K$ as
\begin{align*}
    \regret(K) &\lessapprox
    \sum_{s,a} \min_{t \in [K_{(s,a)}]} \curl*{
    \frac{\Vcal^*(s,a)\log\left(\frac{M}{\delta}\right)\log\left(\frac{\Vcal^*(s,a) \log(M/\delta)}{\gap(s,a) \vee \epsilon_{t}(s,a)}\right)}{\gap(s,a) \vee \epsilon_{t}(s,a)}+ \sqrt{\Vcal^*(s,a) (K_{(s,a)} - t)} } \log(K)\\
    &\qquad + S^2AH^4\log\left(\frac{MK}{\delta}\right)\log\left(\frac{MH}{\returngap_{\min}}\right),
    %O\Bigg(\log(K)\max_{\pi_{1:K}}\min_{\pi^*_{1:K}}\sum_{(s,a) \in \Scal\times\Acal} \min_{t\in %[K]}\Bigg\{\frac{\Vcal_{\max_t}(s,a)}{\breve \gap_{\pi_t}^{\pi^*_t}(s,a)} + %\sum_{k=t+1}^K\frac{\Vcal_{\max_k}(s,a)}{\sum_{j=t+1}^k \breve %\gap_{\pi_j}^{\pi^*_j}(s,a)}\Bigg\}\Bigg).
\end{align*}
where $M\leq (SAH)^3$, $\returngap_{\min} = \min_{(s,a)}\returngap(s,a)$ and $K_{(s,a)}$ is the last episode during which a policy that may visit $(s,a)$ was played. 
% where we only show terms with (inverse-)polynomial dependency on gaps  For the full bound, see \pref{thm:reg_bound_gen_se} in the appendix.
\end{theorem}
%\tm{Possibly state the full version of the result here as we already have an informal version above.}
A slightly more refined version of this bound is stated \pref{thm:reg_bound_gen_se} in \pref{app:upper_bounds}.
Note that our regret bound depends through $\epsilon_{t}(s,a)$, the average gap encountered by $\pi_t$, on the policies that the algorithm played. We can smoothly interpolate between the worst-case rate of $\sqrt{K}$ achieved for $t \ll K$ when all gaps and average gaps are $O(\sqrt{\Vcal^*(s,a) K})$ and the gap-dependent regret rate achieved when $t \approx K$ that scales inversely with gaps. Our bound depends on the gaps in all episodes and can benefit from choices for $t$ that yields a large gap or average gap in late episodes.

